Exploiting Side Information for Improved Online Learning Algorithms in Wireless Networks

In wireless networks, the rate achieved depends on factors like level of interference, hardware impairments, and channel gain. Often, instantaneous values of some of these factors can be measured, and they provide useful information about the instantaneous rate achieved. For example, higher interference implies a lower rate. In this work, we treat any such measurable quality that has a non-zero correlation with the rate achieved as side-information and study how it can be exploited to quickly learn the channel that offers higher throughput (reward). When the mean value of the side-information is known, using control variate theory we develop algorithms that require fewer samples to learn the parameters and can improve the learning rate compared to cases where side-information is ignored. Specifically, we incorporate side-information in the classical Upper Confidence Bound (UCB) algorithm and quantify the gain achieved in the regret performance. We show that the gain is proportional to the amount of the correlation between the reward and associated side-information. We discuss in detail various side-information that can be exploited in cognitive radio and air-to-ground communication in $L-$band. We demonstrate that correlation between the reward and side-information is often strong in practice and exploiting it improves the throughput significantly.

==> ControlVariates.tex <==
%!TEX root =  main.tex


%The control variates is one of the variance reduction methods \citep{JORS85_james1985variance, Willy14_botev2014variance} used in Monte Carlo methods. 
Let $\mu$ be the unknown quantity that needs to be estimated, and $X$ be an unbiased estimator of $\mu$, i.e., $\EE{X} = \mu$. A random variable $W$ is a CV if its expectation $\omega$ is known and it is correlated with $X$. Linear control methods use errors in estimates of known random variables to reduce error in estimation of unknown random variable. For any choice of a coefficient $\beta$, define a new  estimator as
$
    \bar{X} = X + \beta(\omega-W).
$
% is an unbiased estimator of $\mu$ $\bar{X}$ as  $\EE{\bar{X}}=\mu$. and can be easily shown as follows:
% \als{
%     \EE{\bar{X}} &= \EE{X + \beta(\omega-W)}\\
%     &= \EE{X} + \beta\EE{(\omega-W)} \\
%     &= \mu + \beta(\omega - \omega) \\
%     \implies &\EE{\bar{X}} = \mu.
% }
It is straightforward to verify that its variance is given by
\al{
    \text{Var}(\bar{X}) %&= \text{Var}(X) + \beta^2\text{Var}(\omega-W) + 2\beta\text{Cov}(X,\omega- W) \nonumber \\ 
    &= \text{Var}(X) + \beta^2\text{Var}(W) - 2\beta\text{Cov}(X,W).  \label{equ:varNewEst}
}
and is minimized by setting $\beta$ to 
\eq{
    \label{equ:optimalBeta}
    \beta^\star = \frac{\text{Cov}(X,W)}{\text{Var}(W)}.
}
The minimum value of the variance is given by $\text{Var}(\bar{X}) = (1 - \rho^2)\text{Var}(X)$,
% \als{
%     \text{Var}(\bar{X}) &= \text{Var}(X) + \frac{\text{Cov}(X,W)^2}{\text{Var}(W)} - \frac{2\text{Cov}(X,W)^2}{\text{Var}(W)} \\
%     &= \text{Var}(X) - \frac{\text{Cov}(X,W)^2}{\text{Var}(W)} \\
%     &= \text{Var}(X) - \frac{\text{Cov}(X,W)^2}{\text{Var}(X)\text{Var}(W)}\text{Var}(X) \\
%     \implies \text{Var}(\bar{X}) &= (1 - \rho^2)\text{Var}(X),
% }
where $\rho$ is the correlation coefficient of $X$ and $W$. Larger the correlation, the greater the variance reduction achieved by the CV. In practice, the values of $\text{Cov}(X,W)$ and $\text{Var}(W)$ are unknown and need to be estimated to compute the best approximation for $\beta^\star$.


